System-level thermal and electrical modeling of battery systems for electric aircraft design

This work introduces a framework for simulating the electrical power consumption of an 8-seater electric aircraft equipped with high-energy-density NMC Lithium-ion cells. We propose an equivalent circuit model (ECM) to capture the thermal and electrical battery behavior. Furthermore, we assess the need for a battery thermal management system (BTMS) by determining heat generation at the cell level and optimize BTMS design to minimize energy consumption over a predefined flight regime. The proposed baseline battery design includes a 304-kWh battery system with BTMS, ensuring failure redundancy through two parallel switched battery banks. Simulation results explore the theoretical flight range without BTMS and reveal advantages in increasing battery capacity under specific conditions. Optimization efforts focus on BTMS design, highlighting the superior performance of water cooling over air cooling. However, the addition of a 9.9 kW water-cooled BTMS results in a 16.5% weight increase (387 kg) compared to no BTMS, reducing the simulated range of the aircraft from 480 km to 410 km. Lastly, we address a heating-induced thermal runaway scenario, demonstrating the robustness of the proposed battery design in preventing thermal runaway.

==> Sections/Acknowledgement.tex <==
\section{Acknowledgement}\label{sec:acknowledgement}
I would like to express my gratitude to my supervisor, Dr. Ir. Theo Hofman, for providing guidance, feedback, and valuable advice throughout the project. I also extend my thanks to Bernd Rietberg and Tony Bishop for engaging in productive brainstorming sessions and contributing innovative ideas to the realm of electric flight whenever the opportunity arose. Their extensive knowledge of the matter allowed me to surpass my expectations. Special appreciation goes to Jorn van Kampen for diligently proofreading this thesis and providing constructive feedback. Lastly, I want to thank Saurav Sureka and Wouter Andriesse for the support and contribution to the positive work environment in the office.


==> Sections/Appendices.tex <==
\newpage
\section*{Appendix A: Cell specific heat capacity estimation}\label{sec:AppendixA}

Estimating the specific heat capacity of the battery cell is performed over a constant current discharge of 600 seconds. We assume that the energy lost escapes purely as Joule heat and we apply Joule's Law as
\begin{equation}
    P_\mathrm{joule} \approx I_\mathrm{cell}^2\cdot R_0
\end{equation}
where $I_\mathrm{cell}$ is the discharge current and $R_0$ is the internal battery resistance. During the 600 s discharge, we model the consumed energy as
\begin{equation}
    {Q}(t) = -\int_{0}^{600}U_\mathrm{cell}(t)\cdot I_\mathrm{cell}(t)~\mathrm{d}t
\end{equation}
where $U_\mathrm{cell}(t)$ is the cell's voltage. Next, we estimate the specific heat with
\begin{equation}
    c_\mathrm{p} = \frac{Q}{m_\mathrm{cell}\cdot(T_\mathrm{end}-T_0)},
\end{equation}
where $m_\mathrm{cell}$ is the cell's mass, and $T_\mathrm{end}-T_0$ define the temperature difference of the cell. For the NMC in this work, this results in a $c_\mathrm{p}$ value of 1035 J/kg$\cdot$K.

\section*{Appendix B: HPPC test protocol}
At each 10\% state of charge increment, we start a pulse consisting of discharge, rest, and charge. The test assumes that the SOC does not change within the HPPC window at every pulse increment. The followed steps are as follows:
\begin{enumerate}
    % \item Discharge pulse at 1C for 10 seconds.
    % \item Rest for 40 seconds.
    % \item Charge pulse at 0.75C for 10 seconds.
    % \item Rest for 30 minutes.
    % \item Rest for 1 hour.
    % \item new
    \item Standard Constant Current - Constant Voltage (CCCV) charge to $U_\mathrm{cell,max}$.
    \item Rest for 1 hour.
    \item Constant Current (CC) discharge at 1 $\mathrm{C}$ for 30 seconds.
    \item Rest for 40 seconds.
    \item Charge pulse at 0.75 $\mathrm{C}$ for 10 seconds.
    \item Discharge at 1 $\mathrm{C}$ for 6 minutes.
    \item Rest for 1 hour.
    \item Repeat steps (3) - (7) 10 times.
\end{enumerate}
\vspace{12pt}


\begin{table}[ht]
\section*{Appendix C}
\centering
\caption{Aircraft and powertrain parameters and requirements.}
\label{tab:aircraftpara}
% \resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{l|l|c|l}
Symbol &  Property               &  Value   &  Units \\ \hline
  &   &   &  \vspace{-7pt} \\ 
    $m_\mathrm{empty}$  &  Empty aircraft mass &     1489     &kg        \\
    $m_\mathrm{max}$  &  Maximum aircraft mass &     3000     &kg        \\
      $S_\mathrm{w}$ &  Wing area              &  20.8        &  m$^2$      \\
      $C_\mathrm{l}$ &  Lift coefficient       &    0.85      &  -      \\
$C_\mathrm{d}$ & Drag coefficient        & 0.03            &  -\\
$\alpha_\mathrm{max}$ & Maximum angle of attack & 4           & $^\circ$ \\
$\gamma_\mathrm{max}$ & Maximum flight path angle & 8           & $^\circ$ \\
$\gamma_\mathrm{min}$ & Minimum flight path angle & -1           & $^\circ$ \\
$n_\mathrm{m}$ & Number of motors        &  2           & - \\
$P_\mathrm{m,max}$ & Maximum motor power     &   250        & kW \\
$\eta_\mathrm{p}$ & Propeller efficiency    &   0.71          & -\\
 $\omega_\mathrm{p,cons}$& Constant propeller speed    & 4000 & rpm\\
 $\zeta_{\mathrm{b,max}}$ & Maximum SOC    &  1          & - \\
   $\zeta_{\mathrm{b,min}}$ &  Minimum SOC    &  0.15           & - \\
      $P_{\mathrm{aux}}$ &  Auxiliary power consumption    &  4           & kW \\
       % $s_\mathrm{min}$  & Minimal flight range    &  400           & km \\
\end{tabular}%
% }
\end{table}


\begin{table}[ht]
\section*{Appendix D}
\centering
\caption{Cell parameters.}
\label{tab:cellpara}
% \resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{l|l|c|l}
Symbol              & {\color[HTML]{000000} Property}               & {\color[HTML]{000000} Value} & {\color[HTML]{000000} Units}    \\ \hline
&   &   &  \vspace{-6pt} \\ 
$Q_\mathrm{cell}$   & {\color[HTML]{000000} Capacity}               & {\color[HTML]{000000} 11.84} & {\color[HTML]{000000} Ah}       \\
$U_\mathrm{cell,max}$    & {\color[HTML]{000000} Maximum voltage}        & {\color[HTML]{000000} 4.2}   & {\color[HTML]{000000} V}        \\
$U_\mathrm{cell,nom}$    & {\color[HTML]{000000} Nominal voltage}        & {\color[HTML]{000000} 3.4}   & {\color[HTML]{000000} V}        \\
$U_\mathrm{cell,min}$    & {\color[HTML]{000000} Minimum voltage}        & {\color[HTML]{000000} 2.5}   & {\color[HTML]{000000} V}        \\
$I_\mathrm{ch,max}$ & {\color[HTML]{000000} Maximum charge current} & {\color[HTML]{000000} 2.32}  & {\color[HTML]{000000} A}        \\
$I_\mathrm{dis,max}$ & {\color[HTML]{000000} Maximum discharge current}  & {\color[HTML]{000000} 34.8} & {\color[HTML]{000000} A}     \\
$T_\mathrm{cell,min}$    & {\color[HTML]{000000} Minimum temperature}    & {\color[HTML]{000000} -20}   & {\color[HTML]{000000} $^\circ$C} \\
$T_\mathrm{cell,max}$    & {\color[HTML]{000000} Maximum temperature}    & {\color[HTML]{000000} 55}    & {\color[HTML]{000000} $^\circ$C} \\
$T_\mathrm{cell,opt}$    & {\color[HTML]{000000} Optimal temperature range}    & {\color[HTML]{000000} [15,35]}    & {\color[HTML]{000000} $^\circ$C} \\
$m_\mathrm{cell}$    & {\color[HTML]{000000} Cell mass} & {\color[HTML]{000000} 0.103}  & {\color[HTML]{000000} kg} \\
$\rho_\mathrm{GED}$    & {\color[HTML]{000000} Gravimetric energy density} & {\color[HTML]{000000} 390}  & {\color[HTML]{000000} Wh/kg} \\
$c_\mathrm{p}$    & {\color[HTML]{000000} Specific heat capacity} & {\color[HTML]{000000} 1035}  & {\color[HTML]{000000} J/(kg$\cdot$K)} \\
$\operatorname{Bi}$    & {\color[HTML]{000000} Biot number} & {\color[HTML]{000000} 0.0367}  & {\color[HTML]{000000} -} \\
\end{tabular}%
% }
\end{table}



\begin{table}[ht]
\section*{Appendix E}
\centering
\caption{Applied BTMS values.}
\label{tab:BTMSval}
\resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{l|l|c|c|l}
Symbol              & {\color[HTML]{000000} Property}               & {\color[HTML]{000000} Value air} & {\color[HTML]{000000} Value water} & {\color[HTML]{000000} Units}    \\ \hline
      &   &   &   &  \vspace{-6pt} \\ 
$T_\mathrm{fl,in}$   & {\color[HTML]{000000} Inlet temperature}               & {\color[HTML]{000000} 20}  & {\color[HTML]{000000} 20}& {\color[HTML]{000000}$^\circ$C}       \\
$w_\mathrm{ch}$ & {\color[HTML]{000000} Channel width} & {\color[HTML]{000000} $3 \cdot 10^{-3}$} & {\color[HTML]{000000} $3 \cdot 10^{-3}$} & {\color[HTML]{000000} m} \\
$\dot{V}_\mathrm{fl,max}$    & {\color[HTML]{000000} Maximum flow rate}        & {\color[HTML]{000000} 0.0625}& {\color[HTML]{000000} 0.0045}    & {\color[HTML]{000000} m$^3$/s}        \\
$\nu_\mathrm{fl}$ & {\color[HTML]{000000} Kinematic viscosity} & {\color[HTML]{000000} $1.48 \cdot 10^{-5}$} & {\color[HTML]{000000} $1.002 \cdot 10^{-6}$} & {\color[HTML]{000000} m$^2$/s} \\
$k_\mathrm{fl}$    & {\color[HTML]{000000} Thermal conductivity}        & {\color[HTML]{000000} 30} & {\color[HTML]{000000} 600}   & {\color[HTML]{000000} W/K}        \\
$\rho_\mathrm{fl}$    & {\color[HTML]{000000} Density}        & {\color[HTML]{000000} 1.292} & {\color[HTML]{000000} 1000}  & {\color[HTML]{000000} kg/m$^3$}        \\
$c_\mathrm{p,fl}$    & {\color[HTML]{000000} Specific heat capacity}        & {\color[HTML]{000000} 1006}  & {\color[HTML]{000000} 4182}  & {\color[HTML]{000000} J/kg$\cdot$K}        \\
$\operatorname{Pr}$    & {\color[HTML]{000000} Prandtl number}         & {\color[HTML]{000000} 0.71} & {\color[HTML]{000000} 6.9}  & {\color[HTML]{000000} -}        \\
$l$ & Cooling channel length & 1.6 &1.6&m
\end{tabular}%
}
\end{table}



\begin{table}[ht]
\section*{Appendix F}
\centering
\caption{Battery system parameters without BTMS.}
\label{tab:batpara}
\resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{l|l|c|l}
Symbol & {\color[HTML]{000000} Property}              & {\color[HTML]{000000} Value} & {\color[HTML]{000000} Units}       \\ %\hline
\hline & & \\[-2ex]%!!!!!!!!!!!! 
       $U_\mathrm{b}$&Nominal battery system voltage&401.2&V\\
        $Q_\mathrm{b}$&Battery system capacity&304&kWh\\
       $m_\mathrm{b}$& \begin{tabular}[c]{@{}l@{}}Total battery system mass\\ \textit{(including 10\% cell-to-system weight)}\end{tabular} & {\color[HTML]{000000} 856}   & {\color[HTML]{000000} kg}          \\
       $\rho_\mathrm{GED,b}$ & \begin{tabular}[c]{@{}l@{}}Battery system energy density\\ \textit{(including 10\% cell-to-system weight)}\end{tabular} &  355&Wh/kg \\
      $P_\mathrm{b,max,dis}$& {\color[HTML]{000000} Maximum discharge power}        &912 & {\color[HTML]{000000} kW} \\
   $n_\mathrm{p}$ & {\color[HTML]{000000} Number of parallel cells}                       &  {\color[HTML]{000000} 64}     & {\color[HTML]{000000} -}\\
        $n_\mathrm{s}$& {\color[HTML]{000000} Number of series cells}                       &  {\color[HTML]{000000} 118}     & {\color[HTML]{000000} -} \\
        $\Delta T_\mathrm{cell,max}$&\begin{tabular}[c]{@{}l@{}}Maximum cell temperature\\difference in system\end{tabular}&5&$^\circ$C
\end{tabular}%
}
\end{table}



% \begin{figure}[h]
% \section*{Appendix G}
%     \centering
%     \includegraphics[width=0.9\linewidth]{Figures/ThermalNodes2.pdf}
%     \caption{Schematic representation of cells within thermo-electrical network.}
%     \label{fig:ThermalNodes}
% \end{figure}



\begin{figure}[h]
\section*{Appendix G}
    \centering
    \includegraphics[width=0.99\linewidth]{Figures/ThermalModeling3.pdf}
    \caption{Cell vs. system modeling framework.}
    \label{fig:ThermalModeling}
\end{figure}

==> Sections/AppendicesEXT.tex <==
\onecolumn
\section*{External appendices}\label{ch:AppExt}

\subsection{\ul{General cell parameters for 11.84 Ah NMC cell}}

\begin{table}[h]
\centering
% \resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{l|l|l|l}
Symbol              & {\color[HTML]{000000} Property}               & {\color[HTML]{000000} Value} & {\color[HTML]{000000} Units}    \\ \hline
-   & {\color[HTML]{000000} Cell chemistry}               & {\color[HTML]{000000} NMC} & {\color[HTML]{000000}-}       \\
$Q_\mathrm{cell}$   & {\color[HTML]{000000} Capacity}               & {\color[HTML]{000000} 11.84} & {\color[HTML]{000000} Ah}       \\
$U_\mathrm{max}$    & {\color[HTML]{000000} Maximum voltage}        & {\color[HTML]{000000} 4.2}   & {\color[HTML]{000000} V}        \\
$U_\mathrm{max}$    & {\color[HTML]{000000} Nominal voltage}        & {\color[HTML]{000000} 3.4}   & {\color[HTML]{000000} V}        \\
$U_\mathrm{max}$    & {\color[HTML]{000000} Minimum voltage}        & {\color[HTML]{000000} 2.5}   & {\color[HTML]{000000} V}        \\
$I_\mathrm{ch,max}$ & {\color[HTML]{000000} Maximum charge current} & {\color[HTML]{000000} 2.32}  & {\color[HTML]{000000} A}        \\
$I_\mathrm{dis,max}$ & {\color[HTML]{000000} Maximum discharge current}  & {\color[HTML]{000000} 34.8} & {\color[HTML]{000000} A}     \\
$T_\mathrm{min}$    & {\color[HTML]{000000} Minimum temperature}    & {\color[HTML]{000000} -20}   & {\color[HTML]{000000} $^\circ$C} \\
$T_\mathrm{max}$    & {\color[HTML]{000000} Maximum temperature}    & {\color[HTML]{000000} 55}    & {\color[HTML]{000000} $^\circ$C} \\
$\rho_\mathrm{VED}$    & {\color[HTML]{000000} Volumetric energy density}  & {\color[HTML]{000000} 797}  & {\color[HTML]{000000} Wh/l}  \\
$e_\mathrm{cell}$    & {\color[HTML]{000000} Specific energy}  & {\color[HTML]{000000} 1407.0}  & {\color[HTML]{000000} J/kg}  \\
$m_\mathrm{cell}$    & {\color[HTML]{000000} Cell mass} & {\color[HTML]{000000} 103.0}  & {\color[HTML]{000000} g} \\
$\rho_\mathrm{GED}$    & {\color[HTML]{000000} Gravimetric energy density} & {\color[HTML]{000000} 390}  & {\color[HTML]{000000} Wh/kg} \\
$l_\mathrm{cell}$    & {\color[HTML]{000000} Cell length} & {\color[HTML]{000000} 139.0}  & {\color[HTML]{000000} mm} \\
$h_\mathrm{cell}$    & {\color[HTML]{000000} Cell height} & {\color[HTML]{000000} 54.2}  & {\color[HTML]{000000} mm} \\
$w_\mathrm{cell}$    & {\color[HTML]{000000} Cell width} & {\color[HTML]{000000} 6.7}  & {\color[HTML]{000000} mm} \\
$c_\mathrm{p}$    & {\color[HTML]{000000} Specific heat capacity} & {\color[HTML]{000000} 1035}  & {\color[HTML]{000000} J/(kg$\cdot$K)} \\
$k$    & {\color[HTML]{000000} Thermal conductivity} & {\color[HTML]{000000} 26.5}  & {\color[HTML]{000000} W/(m$\cdot$K}) \\
% $h$    & {\color[HTML]{000000} Convective heat transfer coefficient} & {\color[HTML]{000000} \hl{xx}}  & {\color[HTML]{000000} W/(m$^2\cdot$K)} \\
\end{tabular}%
% }
\end{table}



\subsection{\ul{Figure: Cell ECM parameters obtained from HPPC fit}}

\begin{figure}[h]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/R_Values_SA03.eps}
  \caption{ECM resistance values}
  \label{fig:Rval}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/C_Values_SA03.eps}
  \caption{ECM capacitance values}
  \label{fig:Cval}
\end{subfigure}
% \caption{A figure with two subfigures}
\label{fig:RCvalues}
\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\linewidth]{Figures/R_Values_SA03.eps}
%     \label{fig:R}
% \end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\linewidth]{Figures/C_Values_SA03.eps}
%     \label{fig:C}
% \end{figure}


\subsection{\ul{Figure: Battery discharge curve under different C-rates (specified by manufacturer)}}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/SA03_Crates.eps}
    \label{fig:crates}
\end{figure}



\subsection{\ul{Flight profile sequence}}

% \subsection{\ul{Worst-case scenario: maximum power at low SOC}}

\subsection{\ul{Motor datasheet and efficiency map}}

% \subsection{\ul{Pump datasheet}}

% \subsection{\ul{Thermal runaway data fit}}


% \newpage
% \subsection{\ul{Code}}
% \begin{lstlisting}[style=Matlab-editor, basicstyle=\tiny]
% clc
% % close all
% % clear all
% clearvars t time
% % load load_cycles/load_cycle.mat

% BatPara = config.BatPara;
% SysPara = config.SysPara;

% %% Sim_battery_system in code
% dt                  = 1;%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%0.02
% ns                  = SysPara.s_sys;% 3;
% np                  = SysPara.p_sys;% 6;
% startSOC            = 0.98;
% U_cell_start        = 4.135;        % 4.184;%11.88/3;

% Balancing.R         = SysPara.Balancing.R;      %33/np %% 33 Ohms
% Balancing.I_limit   = SysPara.Balancing.I_Limit;
% Balancing.U_delta   = SysPara.Balancing.U_Delta;
% Balancing.U_limit   = SysPara.Balancing.U_Limit;
% Balancing.t_start   = SysPara.Balancing.t_Start;

% m_cell              = BatPara.physical.m;
% cp_cell             = BatPara.thermal.c;
% A_cell              = BatPara.physical.A; % m2
% EnCo                = BatPara.thermal.EnCo;
% U_hys_enable        = 0;
% K_transfer          = results.SysPara.thermal.transfer.K_transfer;%SysPara.thermal.transfer.K_transfer;

% %% Cell parameters for 2RC Lookup tables 
% C_cell              = BatPara.electrical.C_A; %11;%Ah!!!
% T_amb               = 20;
% alpha_cell_ambient(:,:,1)      = 0*ones(np,ns);%5;%SysPara.thermal.alpha_cell_ambient;%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T_cell_ambient(:,:,1)      = 25*ones(np,ns);%results.SysPara.thermal.T_cell_ambient;%SysPara.thermal.T_cell_ambient;

% %% Create Parameter lookup grids (griddedInterpolant)
% %BatPara.electrical.dyn.R_0 %11x2x2: 11_soc*2_T*2_crate, but one dimension can be removed
% SOC_range           = BatPara.electrical.dyn.SOC;%0:0.1:1;
% T_range             = [25, 25.01];
% C_rate_range        = [-1,1];

% % R0_range          = squeeze(BatPara.electrical.dyn.R_0(:,1,:)); %remove 3rd dimension
% R0_range            = BatPara.electrical.dyn.R_0;
% R1_range            = BatPara.electrical.dyn.R1;
% C1_range            = BatPara.electrical.dyn.C1;
% R2_range            = BatPara.electrical.dyn.R2;
% C2_range            = BatPara.electrical.dyn.C2;

% % grid everything, or use interp2
% [SOCgrid,Tgrid,Cgrid] = ndgrid(SOC_range,T_range,C_rate_range); % create ndgrid
% R0_grid = griddedInterpolant(SOCgrid,Tgrid,Cgrid,R0_range);
% R1_grid = griddedInterpolant(SOCgrid,Tgrid,Cgrid,R1_range);
% C1_grid = griddedInterpolant(SOCgrid,Tgrid,Cgrid,C1_range);
% R2_grid = griddedInterpolant(SOCgrid,Tgrid,Cgrid,R2_range);
% C2_grid = griddedInterpolant(SOCgrid,Tgrid,Cgrid,C2_range);

% SOC_OCV_range   = BatPara.electrical.OCV.SOC;
% OCV_range       = BatPara.electrical.OCV.U;
% OCV_grid        = griddedInterpolant(SOC_OCV_range,OCV_range);

% U_hys_max_range = BatPara.electrical.OCV.U_hyst;
% U_hys_max_grid  = griddedInterpolant(SOC_OCV_range,U_hys_max_range);

% %% Preallocations
% I_cell(:,:,1)      = 0*ones(np,ns);
% SOC(:,:,1)         = min(max((startSOC + (0.005*randn(np,ns))), 0), 0.99);
% % SOC(:,:,1)         = startSOC*ones(np,ns);
% C_rate_cell(:,:,1) = 0*ones(np,ns);
% time(:,:,1)        = 0*ones(np,ns);
% U_hys(:,:,1)       = 0*ones(np,ns);
% U_RC1(:,:,1)       = 0*ones(np,ns);
% U_RC2(:,:,1)       = 0*ones(np,ns);
% I_bal(:,:,1)       = 0*ones(np,ns);
% I_pack(1)          = 0;

% U_cell(:,:,1)       = U_cell_start*ones(np,ns);
% U_pack(1)           = sum(U_cell(1,:,1));
% U_pot(:,:,1)        = 0*ones(np,ns);
% U_RC_sum(:,:,1)     = 0*ones(np,ns);
% U_R(:,:,1)          = 0*ones(np,ns);
% max_T_channel_out(1) = config.BTMSConfig.T_fluid;


% PQ_cell(:,:,1) = 0*ones(np,ns);

% T_cell(:,:,1)      = T_amb*ones(np,ns);
% % T_cell_amb         = T_cell_amb; % taken to be constant over flight cycle, 
% % could change with cooling system integrated
% PQ_cell_irr(:,:,1) = 0*ones(np,ns);
% PQ_cell_rev(:,:,1) = 0*ones(np,ns);
% PQ_ambient(:,:,1)  = 0*ones(np,ns);
% PQ_transfer(:,:,1) = 0*ones(np,ns);

% run('deviations_stat');

% m_cell  = m_cell.*SysPara.DeviationMap.m;
% cp_cell = cp_cell.*SysPara.DeviationMap.c;
% EnCo    = EnCo.*SysPara.DeviationMap.EnCo;




% %% BTMS inputs
% A_x = results.SysPara.thermal.transfer.A_x;
% A_y = results.SysPara.thermal.transfer.A_y;
% A_z = results.SysPara.thermal.transfer.A_z;

% T_fluid = config.BTMSConfig.T_fluid;
% Vdot_BTMS = config.BTMSConfig.Vdot_BTMS;
% BTMSConfig = config.BTMSConfig;

% %% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Functional code, main loop
% load('newCurrent.mat')
% I_load = -newCurrent/2; %*BatPara.electrical.C_A*np;
% t(1) = 0;
% disp('Starting cycle')
% tic
% for i = 2:1:length(I_load)

%     time = (i-1)*dt;
%     t(i) = time;
    
%     %R0_now = R0_grid(SOC,I_cell)
%     R0 = R0_grid(SOC(:,:,i-1),T_cell(:,:,i-1),C_rate_cell(:,:,i-1));
%     R1 = R1_grid(SOC(:,:,i-1),T_cell(:,:,i-1),C_rate_cell(:,:,i-1));
%     C1 = C1_grid(SOC(:,:,i-1),T_cell(:,:,i-1),C_rate_cell(:,:,i-1));
%     R2 = R2_grid(SOC(:,:,i-1),T_cell(:,:,i-1),C_rate_cell(:,:,i-1));
%     C2 = C2_grid(SOC(:,:,i-1),T_cell(:,:,i-1),C_rate_cell(:,:,i-1));
    
%     %% Statistical analysis
%     % disabled, enable if possible
%     R0 = R0.*SysPara.DeviationMap.R_0;
%     R1 = R1.*SysPara.DeviationMap.R1;
%     C1 = C1.*SysPara.DeviationMap.C1;
%     R2 = R2.*SysPara.DeviationMap.R2;
%     C2 = C2.*SysPara.DeviationMap.C2;

%     %% Electric potential for single cell (calculate the voltages)
%     % U_Potential = U_SOC + U_Hysteresis + U_RC1 + U_RC2
%     U_OCV = OCV_grid(SOC(:,:,i-1));
%     % Hysteresis from "Verbrugge, 2007 - Adaptive, multi-parameter battery 
%     % state estimator with optimized time weig
%     % hting factors"
%     U_hys_max   = U_hys_max_grid(SOC(:,:,i-1));
%     U_hys(:,:,i)    = (U_hys(:,:,i-1)+(dt.*I_cell(:,:,i-1).*...
%                         (U_hys_max-(U_hys(:,:,i-1).*sign(I_cell(:,:,i-1)))))).*U_hys_enable;
%     U_RC1(:,:,i)    = ((1-exp(-dt./(R1.*C1))).*R1.*I_cell(:,:,i-1)) +...
%                         (U_RC1(:,:,i-1).*(exp(-dt./(R1.*C1))));
%     U_RC2(:,:,i)    = ((1-exp(-dt./(R2.*C2))).*R2.*I_cell(:,:,i-1)) +...
%                         (U_RC2(:,:,i-1).*(exp(-dt./(R2.*C2))));
%     U_pot(:,:,i)    = U_RC1(:,:,i)+U_RC2(:,:,i)+U_OCV+U_hys(:,:,i);
%     U_RC_sum(:,:,i) = U_RC1(:,:,i)+U_RC2(:,:,i);
        
%     %% Ohmic voltage drop and compensating currents in parallel connections
%     I_pack = I_load(i);
%     U_cell(:,:,i)   = ones(np,1).*((sum(I_bal(:,:,i-1),1)+...
%         I_pack+sum((U_pot(:,:,i)./R0),1))./(sum((1./R0),1)));
%     U_R(:,:,i)      = U_cell(:,:,i)-U_pot(:,:,i);
%     I_cell(:,:,i)   = U_R(:,:,i)./R0;
    
%     %% Cell balancing
%     I_bal(:,:,i) = (-U_cell(:,:,i)/Balancing.R).*...
%         (time>=Balancing.t_start).*...
%         (abs(I_pack)<=Balancing.I_limit).*...33
%         (min(U_cell(:,:,i),[],"all")>=Balancing.U_limit).*...
%         ((U_cell(:,:,i)-min(U_cell(:,:,i),[],"all"))>Balancing.U_delta);
%         U_pack(i) = sum(U_cell(1,:,i));%Select and sum rows(series cells)
    
%     %% C-rate and SOC
%     C_rate_cell(:,:,i) = I_cell(:,:,i)/(C_cell*1);
%     delta_SOC = (I_cell(:,:,i)*dt)/(C_cell*3600);
%     SOC(:,:,i) = SOC(:,:,i-1) + delta_SOC;
    
%     %% Thermal model    
%     % Irreversible
%     % PQ_Cells,rev = - I_cell * T_cell * (dUocv/dT_cell) = - I_cell * T_cell * EnCo
%     % Eddahech et al (2013) Thermal characterization of a high-power
%     % lithium-ion battery
%     PQ_cell_irr(:,:,i) = abs(I_cell(:,:,i).*(U_RC_sum(:,:,i)+U_R(:,:,i)));
%     % Reversible
%     PQ_cell_rev(:,:,i) = -(I_cell(:,:,i).*EnCo.*T_cell(:,:,i-1));
%     PQ_cell(:,:,i) = PQ_cell_rev(:,:,i)+PQ_cell_irr(:,:,i);

%     %% BTMS input
%     % BTMSConfig.T_fluid
%     % BTMSConfig.Vdot_BTMS
%     tic
%     [max_T_channel_out(i), T_cell_ambient(:,:,i), alpha_cell_ambient(:,:,i)] =...
%         create_BTMS_input(T_cell(:,:,i-1), T_fluid, Vdot_BTMS,...
%         BTMSConfig, BatPara, A_x, A_y, A_z, ns, np);
%     toc

%     %% Lumped mass thermal model
%     % For fixed alpha_amb and T_cell_amb, enable code below:
%     % PQ_ambient(:,:,i) = alpha_cell_amb.*A_cell.*(T_cell_ambient-T_cell(:,:,i-1));
%     % T_cell(:,:,i) = T_cell(:,:,i-1)+((dt*(PQ_cell(:,:,i)+PQ_ambient(:,:,i)+...
%     % PQ_transfer(:,:,i-1)))./(m_cell.*cp_cell));
%     PQ_ambient(:,:,i) = alpha_cell_ambient(:,:,i).*A_cell.*(T_cell_ambient(:,:,i)-T_cell(:,:,i-1));
%     T_cell(:,:,i) = T_cell(:,:,i-1)+((dt*(PQ_cell(:,:,i)+PQ_ambient(:,:,i)+...
%         PQ_transfer(:,:,i-1)))./(m_cell.*cp_cell));

%     %% Heat transfer model
%     Heat_transfer = 1; %on/off
%     % K_transfer % Define a function to shape the K matrix
%     % reshape the matrix to display the parallel cells on the rows and series cells in columns.
%     PQ_transfer(:,:,i) = reshape((K_transfer*reshape(T_cell(:,:,i-1),[],1)),np,ns)*Heat_transfer;

    
%     %% Progress bar of model
%     if ~(mod(i,1000))
%     disp([num2str(i/length(I_load)*100),' %'])
%     end
% end
% toc
% return

% %% plots %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Cell State-of-charges
% figure()
% Dim = size(SOC);
% SOC2 = reshape (permute(SOC, [3,2,1]), Dim(3), []);
% plot (SOC2); 
% title('Cell State-of-charges')
% xlabel('Time [s]'); grid on
% return
% %% Battery system current load
% figure()
% plot(t,I_load)
% title('Battery system current load')
% xlabel('Time [s]'); grid on
% %% Battery system voltage
% figure()
% plot(t,U_pack)
% title('Battery system voltage')
% xlabel('Time [s]'); grid on
% %% Cell current loads
% figure()
% Dim = size(I_cell);
% I_cell2 = reshape(I_cell,...
%     [length(I_cell(:,1,1))*length(I_cell(1,:,1)), length(I_cell(1,1,:))]);
% %reshape (permute(I_cell, [3,2,1]), Dim(3), []);
% plot (I_cell2); 
% title('Cell current loads')
% xlabel('Time [s]'); grid on
% %% Cell voltages
% figure()
% Dim = size(U_cell);
% U_cell2 = reshape (permute(U_cell, [3,2,1]), Dim(3), []);
% plot (U_cell2); 
% title('Cell voltages')
% xlabel('Time [s]'); grid on
% %% Cell State-of-charges
% figure()
% Dim = size(SOC);
% SOC2 = reshape (permute(SOC, [3,2,1]), Dim(3), []);
% plot (SOC2); 
% title('Cell State-of-charges')
% xlabel('Time [s]'); grid on
% %% Cell ECM sum
% figure()
% Dim = size(U_RC_sum);
% U_RC_sum2 = reshape (permute(U_RC_sum, [3,2,1]), Dim(3), []);
% plot (U_RC_sum2); 
% title('Cell ECM sum')
% xlabel('Time [s]'); grid on
% %% Cell ohmic voltage drops
% figure()
% Dim = size(U_R);
% U_Rb = reshape (permute(U_R, [3,2,1]), Dim(3), []);
% plot (U_Rb); 
% title('Cell ohmic voltage drops')
% xlabel('Time [s]'); grid on
% %% Cell temperatures
% figure()
% Dim = size(T_cell);
% T_cell2 = reshape (permute(T_cell, [3,2,1]), Dim(3), []);
% plot (t,T_cell2); 
% title('Cell temperatures')
% xlabel('Time [s]'); grid on
% hold on
% plot(t,max_T_channel_out)
% %% Ambient heat transfer
% figure()
% Dim = size(PQ_ambient);
% PQ_ambient2 = reshape (permute(PQ_ambient, [3,2,1]), Dim(3), []);
% plot (t,PQ_ambient2); 
% title('Ambient heat transfer')
% xlabel('Time [s]'); grid on

% %% Needed cooling power
% P_cool = -sum(PQ_ambient2');
% plot (P_cool); 

% %% Heat transfer between cells
% figure()
% Dim = size(PQ_transfer);
% PQ_transfer2 = reshape (permute(PQ_transfer, [3,2,1]), Dim(3), []);
% plot (PQ_transfer2); 
% title('Heat transfer between cells')
% xlabel('Time [s]'); grid on

% %% Plot all in 1 figure
% % % figure()
% % % return
% % % %% Plot all in 1 figure
% % % figlist=get(groot,'Children');
% % % newfig = figure;
% % % newfig.WindowState = 'maximized';
% % % tcl=tiledlayout(newfig,'flow');
% % % 
% % % for i = 1:numel(figlist)
% % %     figure(figlist(i));
% % %     ax=gca;
% % %     ax.Parent=tcl;
% % %     ax.Layout.Tile=i;
% % % end
% % % close(figlist)


% %% functions (if needed)
% function [max_T_channel_out, T_cell_ambient, alpha_cell_ambient] = create_BTMS_input(T_cell, T_fluid_BTMS, Vdot_BTMS, BTMSConfig, BatPara, A_x, A_y, A_z, s, p)
%     %% Transform T_cell to column vector
%     T_cell_vec = reshape(T_cell, [numel(T_cell),1]);
%     %% Some necessary variables
%     A_dir = [A_x, A_y, A_z];
%     A_cell_total = BatPara.physical.A;
%     %% Get average temperature of cells adjacent to the cooling channels
%     T_avg_cell_channel = NaN(BTMSConfig.num_channels, 1);
%     for ii = 1:BTMSConfig.num_channels
%         T_avg_cell_channel(ii) = sum(T_cell_vec(nonzeros(BTMSConfig.channel_def_mat(ii,:))'))/BTMSConfig.channel_num_adj_cells(ii);
%     end
%     %% Get volume and mass flow and speed through each cooling channel
%     %% Calculate channel heat transfer coefficient
%     %% Calculate average cooling channel temp
%     T_channel_out = NaN(BTMSConfig.num_channels, 1);
%     for ii = 1:BTMSConfig.num_channels
%         T_channel_out(ii) = get_fluid_out_temp(T_fluid_BTMS, T_avg_cell_channel(ii), BTMSConfig.channel_length(ii), BTMSConfig.channel_mdot(ii), BTMSConfig.fluid_para.cp, BTMSConfig.lambda_wall);
%     end
%     T_channel_avg = (T_fluid_BTMS + T_channel_out) / 2;
    
%     %% Write values is vectors
%     % T_cell_ambient_vec: Meat temperature around each cell
%     % alpha_cell_ambient_vec: Scaled heat transfer coefficient
%     [alpha_cell_ambient_vec, T_cell_ambient_vec]  = cal_output_vecs(T_channel_avg, BTMSConfig.channel_alpha, BTMSConfig.channel_def_mat, BTMSConfig.channel_orientation, A_dir, A_cell_total, s * p);
    
%     %% Recreate matrix structure for sim_battery_system
%     T_cell_ambient = reshape(T_cell_ambient_vec, [p, s]);
%     alpha_cell_ambient = reshape(alpha_cell_ambient_vec, [p, s]);
%     max_T_channel_out = max(T_channel_out);
% end

% function T_channel_out = get_fluid_out_temp(T_channel_in, T_avg_cell, channel_length, mdot, c_p_fluid, lambda_wall)
%     % Calculate approximated channel output temperature
%     % Approximation for axial flow in pipe
%         epsilon = lambda_wall / (mdot * c_p_fluid);
%     T_channel_out = (T_channel_in - T_avg_cell) * exp(-epsilon*channel_length) + T_avg_cell;  
        
% end

% function [alpha_cell_ambient_vec, T_cell_ambient_vec]  = cal_output_vecs(T_channel_avg, alpha_channel, channel_def_mat, channel_orientation, A_dir, A_cell_total, number_of_cells)
    
%     % Preallocate output vectors
%     alpha_cell_ambient_vec = zeros(1, number_of_cells);
%     T_cell_ambient_vec = zeros(1, number_of_cells);
    
%     for ii = 1:number_of_cells
        
%         % Look if a cell is adjacent to one or more cooling channels
%         [row, ~] = find(channel_def_mat == ii);
%             if length(row) >= 1     % Cell is in contact with one or more cooling channels
                
%                 % Calculate mean temperature around cell
%                 T_cell_ambient_vec(ii) = sum(T_channel_avg(row)) / length(row);
                
%                 % Get vector with area of heat transfers
%                 A_heat_total_cell = zeros(length(row), 1);
                
%                 x_dir = find(channel_orientation(row) == 'x');
%                 y_dir = find(channel_orientation(row) == 'y');
%                 z_dir = find(channel_orientation(row) == 'z');
                
%                 A_heat_total_cell(x_dir) = A_dir(1);
%                 A_heat_total_cell(y_dir) = A_dir(2);
%                 A_heat_total_cell(z_dir) = A_dir(3);
                
%                 % Calculate scaled heat transfer coefficient
                
%                 % The alpha value computed here will get multiplied with the total cell
%                 % surface in the simulation model --> We must scale the heat transfer
%                 % coefficient to the total cell surface.
    
%                 % Example for a cell that is cooled from both x-sides and from one y-side:
%                 % alpha_total = (alpha_x1*A_x + alpha_x2*A_x + alpha_y*A_y) / A_cell
                
%                 alpha_cell_ambient_vec(ii) = sum(alpha_channel(row) .* A_heat_total_cell) / A_cell_total;
            
%             end
%     end
% end


% \end{lstlisting}


